RoPAWS: Robust Semi-supervised Representation Learning from Uncurated Data

Semi-supervised learning aims to train a model using limited labels. State-of-the-art semi-supervised methods for image classification such as PAWS rely on self-supervised representations learned with large-scale unlabeled but curated data. However, PAWS is often less effective when using real-world unlabeled data that is uncurated, e.g., contains out-of-class data. We propose RoPAWS, a robust extension of PAWS that can work with real-world unlabeled data. We first reinterpret PAWS as a generative classifier that models densities using kernel density estimation. From this probabilistic perspective, we calibrate its prediction based on the densities of labeled and unlabeled data, which leads to a simple closed-form solution from the Bayes' rule. We demonstrate that RoPAWS significantly improves PAWS for uncurated Semi-iNat by +5.3% and curated ImageNet by +0.4%.

==> backup.tex <==
% Prior works include label propagation~\citep{lee2013pseudo} and regularization~\citep{sajjadi2016regularization,xie2020unsupervised} to utilize unlabeled data.
% These two methods were later combined to generate more accurate pseudo-labels~\citep{berthelot2019mixmatch,berthelot2020remixmatch,sohn2020fixmatch}.
% More
% \tbd{revise this}

% Prior works have attempted to design a better algorithm~\citep{berthelot2019mixmatch,berthelot2020remixmatch,sohn2020fixmatch} by combining the propagation of labels~\citep{lee2013pseudo} and regularization from unlabeled data~\citep{sajjadi2016regularization}.
% Recent works exploit the success of self-supervised learning~\citep{he2020momentum,chen2020simple} in learning representations from unlabeled data for training large-scale semi-supervised models~\citep{chen2020big}. In particular, PAWS~\citep{assran2021semi} proposed a single-stage approach that combines supervised and self-supervised learning and achieves state-of-the-art accuracy and convergence speed.

% methods like
% they are

% \citep{chen2020semi,guo2020safe,yu2020multi,saito2021openmatch,liu2022open}.
% , e.g., unlabeled data contain
% uncertain (confusing in-class) or
% out-of-class data.

% misses the opportunity to learn representations from the OOD data and is ineffective for large-scale realistic datasets.
% OOD filtering can also be inadequate when the OOD samples are not discriminative.


% uncertain (i.e., rare data not covered by labels, often with distribution shifts) or out-of-class data
% Specifically, RoPAWS propagates the labels of nearby labeled and unlabeled data. 
% \jc{Specifically, talk about the uncertain data which are often rare data not covered by labels (OOD), often with distribution shifts... 
% (not using i.e. because there are too many breaks to the readers)}
% To this end, w


% PAWS assigns the pseudo-label of unlabeled data by the nearest labeled data; however, this makes the prediction of out-of-class data overconfident. 
% In uncurated setting, unlabeled data contains out-of-class data, for which the model should have unconfident predictions. Therefore, RoPAWS regularizes the pseudo-labels by comparing the similarities between unlabeled data and labeled data.
% The idea of RoPAWS is to calibrate the prediction of unlabeled data
% by measuring the similarities between \emph{both} labeled and unlabeled data. 
%% Need to rewrite the following 3 sentences
% Here, data far from labeled data has less confident predictions, which again calibrates predictions of nearby unlabeled data. \jc{I don't quite understand this sentence.}
% In contrast, PAWS only considers the nearby labeled data and makes predictions overconfident in known classes.
% Using the calibrated prediction as targets, RoPAWS can be robustly trained under the uncurated data.
% \tbd{revise this paragraph}

% and Figure~\ref{fig:tsne} visualizes the learned representations.


% especially under relatively small datasets~
% does not fully leverage representation learning
% fully leverage the representation of neural networks and
% \footnote{
% Pseudo-labeling (or self-training) also works for large scenarios when the initial supervised model produces reliable pseudo-labels. However, it does not work well when labels are limited, as shown in Table~\ref{tab:sinat}.}

% \revised{with $C_\text{all}$ classes}
% \jc{Can we define $C$ here?}
% \footnote{PAWS adopts the recent techniques of self-supervised learning such as projection/prediction networks and multi-crop augmentation. We omit them and focus on the prediction. See Appendix~\ref{appx:details} for details.}

% \jc{$\{x_l^i,y_l^i\}_N$? same for $B_u$}
% Due to the limitation of resource,
% We sample a subset of classes for each batch if the number of classes is large.
% where $[C]$ is often a subset of the entire classes.
%$[C_\text{all}]$.

% where $[C]$ is a subset of 


% (can be a subset of the entire class $[C_\text{all}]$).\jc{this is little confusing since we only use $C$ in the following context. Maybe say $C_{subset}$? Also don't use the () for this sentence}

% (with super-/sub-scripts).
% a $n$-size batch of embeddings be
% \jc{rewrite this sentence}.
% based on a soft nearest-neighbor classifier, i.e.,
% where $\mathbf{z}_l \in \mathbb{R}^{N \times d}$ are the embeddings of labeled data,

% by uncertainty using density estimation to make PAWS \jc{more robust\st{robustly trained from the uncurated data}}.

% of labeled data
% Our derivation can be also interpreted as a fixed-point solution of the 
% provides an alternative view from the Bayes' rule of the fixed-point solution of the iterative label propagation.

% , where the target is detached\jc{from what?}.


% We verify the effectiveness of RoPAWS under various scenarios. In Section~\ref{subsec:exp-large}, we demonstrate the results on large-scale datasets where representation learning plays a crucial role. In Section~\ref{subsec:exp-small}, we present the results on small-scale datasets and compare RoPAWS with prior robust semi-supervised learning methods. Finally, in Section~\ref{subsec:exp-analysis}, we provide ablation studies and analyses.

% We use the SwAV~\citep{caron2020unsupervised} checkpoint for ImageNet pre-trained models.
% , since it gives a better initialization, as shown in Appendix~\ref{appx:pretrain}.

% We provide the ImageNet~\citep{deng2009imagenet} experiments.
% consists of 1.3M images with 1K classes.
% experiments.
% \jc{\st{the standard benchmark for image classification} this is redundant. Combine with the next sentence.}.
% ImageNet consists of 1.3M images with 1K classes.
% we consider the curated setup

% The original ImageNet-21k consists of 14M images with 21K classes, where a subset of 1M images with 1K classes (called ImageNet-1k) is usually reported.
% Prior work trained a 1K classifier using ImageNet-1k as unlabeled data and its subset (1\% or 10\%) of as labeled data. In addition to this curated setup, we consider the uncurated setup using the same labeled subset of ImageNet-1k but ImageNet-21k as unlabeled data. We compare RoPAWS with PAWS (state-of-the-art), along with MPL~\citep{pham2021meta} and SimCLRv2~\citep{chen2020big} results from the PAWS paper.


% UDA~\citep{xie2020unsupervised}, FixMatch~\citep{sohn2020fixmatch}, MPL~\citep{pham2021meta}, BYOL~\citep{grill2020bootstrap} SwAV~\citep{caron2020unsupervised}, and SimCLRv2~\citep{chen2020big} results from the PAWS paper.

% Table~\ref{tab:sinat} presents the ImageNet results. RoPAWS achieves state-of-the-art accuracy on the standard ImageNet-1k (curated) benchmark, improving PAWS by \tbd{x.x\%} and \tbd{x.x\%} using 1\% or 10\% of labels, respectively. RoPAWS is more impactful for the uncurated scenario of ImageNet-1k (+ ImageNet-21k), improving PAWS by \tbd{x.x\%} and \tbd{x.x\%} using 1\% or 10\% of labels, respectively.
% We also provide the results using a soft nearest-neighbor classifier and using 100\% labels in Appendix~\ref{appx:imagenet}.

% We further provide the results on small-scale datasets. Recall that most prior robust semi-supervised methods assumed the uncurated data consists of in- and out-of-domain (OOD) data and attempted to filter OOD data. In this perspective, they focused on easy OOD setups where the OOD data can be discriminated relatively easily from the in-domain data. Here, we study both easy OOD and hard OOD setups and compare RoPAWS with the prior works in both scenarios.


% nto the interim area
% , i.e., well-calibrated\jc{need better way to describe this}.



% \jc{Say improve PAWS by 5.3\% instead}

% Recently, self-supervised learning greatly advanced learning representations from unlabeled data and improved semi-supervised learning in large-scale scenarios.
% Specifically, PAWS extended the siamese-based self-supervised learning using labels and has shown outstanding results in semi-supervised image classification. 
% To handle this, we propose RoPAWS, a robust extension of PAWS for uncurated data. 
% modeling densities on representation by kernel density estimation. 
% Semi-supervised learning aims to improve the representation by leverage large amount of unlabeled data and a limited amount of annotations. 
% Despite the recent success of semi-supervised methods such as PAWS, they are often when unlabeled data is uncurated, e.g., contains uncertain or out-of-class data. 
% To handle this, we propose RoPAWS, a robust extension of PAWS for uncurated data. To this end, we reinterpret PAWS as a generative classifier modeling densities on representation by kernel density estimation. Using this probabilistic view, we calibrate the prediction based on the densities of labeled and unlabeled data, which leads to a simple closed-form solution from the Bayes rule.
% \revised{We demonstrate that RoPAWS significantly improves PAWS for various datasets, e.g., elevating the state-of-the-art for Semi-iNat by +1.7\% and ImageNet by \tbd{+x.x\%}.}


%% Explain what is Semi-SL, how do they work? What assumptions?
% (Semi-SL)
% The goal of Semi-SL is to leverage large-scale unlabeled data to train models, together with small amount of labeled data.

% Many methods leverage self-supervised learning using a two-stage approach of self-supervised pre-training on the unlabeled data and then fine-tuning on the small labeled data.
% However, recently, 

% Learning with limited labels is a fundamental challenge in machine learning and computer vision.
% Being as one of the most promising direction, semi-supervised learning provide a solution that enables joint learning from (small) labeled and large-scale unlabeled data. 
% The unlabeled data can be leveraged in a variety of different ways\citep{berthelot2019mixmatch,berthelot2020remixmatch,sohn2020fixmatch} including label propagation~\citep{lee2013pseudo} and regularization~\citep{sajjadi2016regularization}.
% learning from data themselves
% , particularly for semi-supervised image classification
% Here, most prior works focused on regularizing the classifier's prediction (i.e., the prediction-based approach), propagating labels
%% Current SOTA methods: heavily biased towards Self-SL methods, two stage (self-SL then fine-tuning) or one-stage? Currently one-stage (PAWS) is the best
% Afterward, many works have attempted to leverage self-supervision for semi-supervised learning~\citep{chen2020big}. 

% The self-supervised representations can also be leveraged for training large-scale semi-supervised models~\citep{chen2020big}.

% RoPAWS is built upon PAWS~\citep{assran2021semi}, the state-of-the-art semi-supervised learning method that leverages the recent success of self-supervision.
% However, PAWS is often prone to uncurated data since it predicts unlabeled data (possibly out-of-class) confidently as the known classes. To handle this issue, RoPAWS calibrates the prediction of PAWS by modeling density over the representation space and makes the training robust using the calibrated prediction.
% The remaining section is as follows.

% We focus on the final formulas and omit most derivations for brevity. See Appendix~\ref{appx:derivation} for detailed derivations.


% PAWS~\citep{assran2021semi} showed a one-stage joint training of supervision and self-supervision achieves state-of-the-art in terms of both accuracy and convergence speed. \tbd{revise}

% While the initial works considered the two-stage approach of self-supervised pre-training and then fine-tuning, PAWS~\citep{assran2021semi} revealed that a one-stage joint training of supervision and self-supervision achieves state-of-the-art in terms of both accuracy and convergence speed.


% In particular, fine-tuning a simple classifier on top of the self-supervised pre-trained models highly outperformed the prediction-based approach, especially for the practical scenarios of high-resolution images with a large amount~\citep{chen2020big}.

% However, this two-stage approach of self-supervised pre-training and then fine-tuning is inefficient when the target downstream task is given. From this motivation, PAWS~\citep{assran2021semi} leverages the labels for representation learning, extending the design of self-supervised learning methods (particularly the siamese network approach~\citep{caron2020unsupervised}) to semi-supervised learning by incorporating the labels in the training objective. As a result, PAWS has shown to be more effective (i.e., better accuracy) yet efficient (i.e., converges faster) than the two-stage approaches.

%% Explain when SOTA methods don't work. Previous methods only experimented on curated datasets, and


% predict the class considering both labeled and unlabeled data, and 
% robust to uncurated data that can leverage labeled
% \tbd{ref to figure 1, give easy intuition (semi-sup)}


% From this probabilistic view, we derive a novel yet simple extension of PAWS.
% The core idea of RoPAWS is to calibrate the prediction
% This probabilistic view provides a principled way to extend PAWS, e.g., considering out-of-class data.
% Our motivation is that PAWS, the state-of-the-art method on (curated) benchmarks, is prone to be overconfident to the known classes and still make incorrect predictions even for out-of-class data in the uncurated dataset.
% uncurated data by making predictions overconfident to the known classes, giving wrong targets for uncertain or out-of-class data. 
% \revised{To this end, our high level ides is to }
% we calibrate the prediction and regularize the training of PAWS through a probabilistic lens.
% Specifically, our main technical contributions are as follows:
% \begin{itemize}[topsep=1.0pt,itemsep=1.0pt,leftmargin=7.5mm]
% \item We suggest a novel interpretation of PAWS as a generative classifier, modeling densities on the representation space by kernel density estimation (KDE)~\citep{rosenblatt1956remarks}. This probabilistic view provides a principled way to extend PAWS, e.g., considering out-of-class data.
% \item We propose RoPAWS, a novel yet simple extension of PAWS. The core idea of RoPAWS is to calibrate the prediction considering the densities of labeled and unlabeled data. Then, the final prediction is given by a closed-form solution from the Bayes rule, which implicitly finds the fixed point of an iterative propagation formula of labels and priors of unlabeled data.
% \item In addition, RoPAWS explicitly controls out-of-class data by modeling prior distribution and assigning reweighted loss, making the model further robust under the uncurated data.
% \item We propose RoPAWS, a novel yet simple extension of PAWS. RoPAWS calibrates the prediction considering the densities of labeled and unlabeled data. The final prediction is given by a closed-form solution from the Bayes rule, which also relates to label propagation.
% \item We further improve RoPAWS by incorporating out-of-class into the prior label distribution and regularizing the prediction of uncertain samples, combined with the reweighted loss.
% \end{itemize}



% Despite the success on well-curated benchmarks, prior semi-supervised learning methods 
% We observed that the accuracy of PAWS significantly drops for these scenarios.
% Some prior works called robust semi-supervised learning aimed to tackle this problem by filtering out-of-distribution (OOD) data~\citep{chen2020semi,yu2020multi,saito2021openmatch,liu2022open}.
% However, the OOD filtering approach ignores the representation learned from OOD data and is ineffective when OOD is not discriminative; they did not report the results on large-scale realistic datasets.

% , and did not show results on realistic large-scale datasets 

% and underperforms when OOD data are not discriminative.

% . Thus, we argue that it is better to utilize OOD data for representation learning.
% to filter out-of-distribution (OOD) samples from the uncurated data, as they are irrelevant to the in-class prediction~\citep{chen2020semi,yu2020multi,saito2021openmatch,liu2022open}. 

% On the other hand, a line of work
% PAWS is often error-prone when the unlabeled data is uncurated, i.e., contains uncertain or out-of-class data. It contrasts with the robustness of self-supervised learning, which learns useful representation from out-of-distribution~\citep{goyal2021self} of even synthetic~\citep{baradad2021learning} data. We aim to bridge the gap between the robustness of self-supervised learning and the efficacy (and efficiency) of semi-supervised learning and extend the applicability of PAWS for realistic uncurated datasets.
% Semi-supervised learning from uncurated data has been widely investigated for the prediction-based approach~\citep{oliver2018realistic}.
% , especially when considering their soft confidence.

% a single-stage% To this end, 



% and RoPAWS outperforms PAWS (SOTA)
% including large-scale datasets such as Semi-iNat~\citep{su2021semi} and ImageNet~\citep{deng2009imagenet}. 

% \jc{have a bar graph here summarizing the results.}
% \jc{add another figure on the architecture of RoPAWS, highlighting that we are treating the OOD (uncertain) and in-domain unlabeled data differently. This figure need to be self-contained, no need to know the details of PAWS.}
% \jc{we can tone down about one stage is better than two stage methods.}

% \begin{itemize}[topsep=1.0pt,itemsep=1.0pt,leftmargin=7.5mm]
% \item RoPAWS improves PAWS by +5.3\% on Semi-iNat, and outperforms the state-of-the-art robust semi-supervised learning method, CCSSL~\citep{yang2022class}, by +1.7\%.
% \item RoPAWS also helps the (curated) benchmarks by calibrating the prediction of uncertain data, e.g. outperforming PAWS (state-of-the-art) by +0.4\% on ImageNet with 1\% labels.
% \item RoPAWS outperforms the prior robust methods, e.g., OpenMatch~\citep{saito2021openmatch} by +5.2\%
% % and OpenCos~\citep{park2021opencos} by +0.6\%
% on CIFAR-10 \citep{krizhevsky2009learning} (+ Tiny-ImageNet) with 25 labels.
% \end{itemize}

==> default_notation.tex <==
\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}
